Application of the Landauer-B\"uttiker method to the calculation of interlayer exchange coupling in closed ballistic multi-layers

In this communication we study the behaviour of spin current components in a ballistic junction consisting of two semi-infinite leads and a scattering region composed of two magnetic layers separated by a non-magnetic metallic spacer. We then consider the system being gradually isolated from the leads, which we refer to as the transition from an open to a closed regime. As expected on physical grounds, charge and in-plane components vanish, but the out-of-plane spin current remains finite and gives rise to the oscillatory interlayer exchange coupling (IEC) between the magnets. We show that the out-of-plane spin current reduces to a set of peaks in momentum space, which correspond to discrete energy eigenstates of the closed system. Furthermore, we demonstrate that the expression for the IEC in terms of spin current for an open system reduces to an expression in the closed system, which corresponds exactly to the definition of IEC in terms of energy difference.

==> potentialProfile1.tex <==
% !TEX root = ../main.tex
\tikzstyle{inc}=[->,shorten <=1pt, >=stealth', semithick] 
\tikzstyle{ref}=[<-,shorten <=1pt, >=stealth', semithick] 
\begin{center} 
\begin{tabular}{cc}
\input{tikz/plot0}
\\
\begin{tikzpicture}[scale=0.6]
\draw[->](-2.5,0)--(10,0)node[below right]{$y$}coordinate(x axis);  
\draw[->](0,-2.5)--(0,3.5)node[above left]{$E$}coordinate(y axis);  
\draw[very thick](-2.5,0)--(0,0)node[below left]{$O$};  
\draw[very thick](8.5,0)--(10,0);  
\draw[dashed](-2.5,1.3)--(10,1.3)node[above right]{$E_{F}$};  
\draw[very thick](0,0)--(0.5,0)--(1,0)--(1,-2)--(3,-2)--(3,0)--(6.5,0)--(6.5,-2)--(8,-2)--(8,0)--(8.5,0);  
\draw[dashed](1,-1.6)--(3,-1.6);  
\draw[dashed](6.5,-1.6)--(8.0,-1.6);  
\end{tikzpicture} 

\end{tabular}
\caption{Potential profile of the standard CPP switching geometry and the plots of the reflection factor $\Delta$ and the out-of-plane spin current density in momentum space as functions of the in-plane momentum magnitude $\kpar$}
\label{fig:profile1}
\end{center}

==> potentialProfile2.tex <==
% !TEX root = ../main.tex
\tikzstyle{inc}=[->,shorten <=1pt, >=stealth', semithick] 
\tikzstyle{ref}=[<-,shorten <=1pt, >=stealth', semithick] 
\begin{center} 
\begin{tabular}{cc}
\input{tikz/plot1}
\\
\begin{tikzpicture}[scale=0.6]
\draw[->](-2.5,0)--(10,0)node[below right]{$y$}coordinate(x axis);  
\draw[->](0,-2.5)--(0,3.5)node[above left]{$E$}coordinate(y axis);  
\draw[very thick](-2.5,0)--(0,0)node[below left]{$O$};  
\draw[very thick](8.5,0)--(10,0);  
\draw[dashed](-2.5,1.3)--(10,1.3)node[above right]{$E_{F}$};  
\draw[very thick](0,0)--(0.5,0)--(0.5,1.2)--(1,1.2)--(1,-2)--(3,-2)--(3,0)--(6.5,0)--(6.5,-2)--(8,-2)--(8,1.2)--(8.5,1.2)--(8.5,0) ;  
\draw[dashed](1,-1.6)--(3,-1.6);  
\draw[dashed](6.5,-1.6)--(8.0,-1.6);  
\end{tikzpicture} 

\end{tabular}
\caption{Potential profile of the standard CPP switching geometry with additional barriers introduced between the magnets and the leads. Varying the heights of the barriers realizes the regime where the system is gradually isolated from the macroscopic reservoirs (connected via leads). Spin current density begins to develop distinct resonances in momentum space. Positions of the resonances correspond to the points where reflection factor $\Delta$ is close to zero.}
\label{fig:profile2}
\end{center}

==> potentialProfile3.tex <==
% !TEX root = ../main.tex
\tikzstyle{inc}=[->,shorten <=1pt, >=stealth', semithick] 
\tikzstyle{ref}=[<-,shorten <=1pt, >=stealth', semithick] 
\begin{center} 
\begin{tabular}{cc}
\input{tikz/plot2}
\\	
\begin{tikzpicture}[scale=0.6] 
\draw[->](-2.5,0)--(10,0)node[below right]{$y$}coordinate(x axis);  
\draw[->](0,-2.5)--(0,3.5)node[above left]{$E$}coordinate(y axis);  
\draw[very thick](-2.5,0)--(0,0)node[below left]{$O$};  
\draw[very thick](8.5,0)--(10,0);  
\draw[dashed](-2.5,1.3)--(10,1.3)node[above right]{$E_{F}$};  
\draw[very thick](0,0)--(0.5,0)--(0.5,4)--(1,4)node[above,midway]{}--(1,-2)--(3,-2)--(3,0)--(6.5,0)--(6.5,-2)--(8,-2)--(8,4)--(8.5,4)node[above,midway]{}--(8.5,0) ;  
\draw[dashed](1,-1.6)--(3,-1.6);  
\draw[dashed](6.5,-1.6)--(8.0,-1.6);  
\end{tikzpicture} 

\end{tabular}
\caption{As the barrier height is increased up to and beyond the Fermi level, the system becomes effectively isolated from the reservoirs and transitions into the \textit{closed} regime. Spin current density collapses into a set of resonances at a set of points in momentum space away from which it vanishes. Positions of the resonances appear to coincide with the zeros of the reflection factor. This is consistent with the model of the closed system described using Landauer formalism.}
\label{fig:profile3}
\end{center}
